$\varepsilon$-fractional Core Stability in Hedonic Games

Hedonic Games (HGs) are a classical framework modeling coalition formation of strategic agents guided by their individual preferences. According to these preferences, it is desirable that a coalition structure (i.e. a partition of agents into coalitions) satisfies some form of stability. The most well-known and natural of such notions is arguably core-stability. Informally, a partition is core-stable if no subset of agents would like to deviate by regrouping in a so-called core-blocking coalition. Unfortunately, core-stable partitions seldom exist and even when they do, it is often computationally intractable to find one. To circumvent these problems, we propose the notion of $\varepsilon$-fractional core-stability, where at most an $\varepsilon$-fraction of all possible coalitions is allowed to core-block. It turns out that such a relaxation may guarantee both existence and polynomial-time computation. Specifically, we design efficient algorithms returning an $\varepsilon$-fractional core-stable partition, with $\varepsilon$ exponentially decreasing in the number of agents, for two fundamental classes of HGs: Simple Fractional and Anonymous. From a probabilistic point of view, being the definition of $\varepsilon$-fractional core equivalent to requiring that uniformly sampled coalitions core-block with probability lower than $\varepsilon$, we further extend the definition to handle more complex sampling distributions. Along this line, when valuations have to be learned from samples in a PAC-learning fashion, we give positive and negative results on which distributions allow the efficient computation of outcomes that are $\varepsilon$-fractional core-stable with arbitrarily high confidence.

==> fig_fhg.tex <==
\begin{figure}[tb!]
\centering
\begin{tikzpicture}[-, line width = 0.5pt]
\tikzset{position/.style args={#1:#2 from #3}{at=(#3.#1), anchor=#1+180, shift=(#1:#2)}}

			%\begin{tikzpicture}

			\def \n {10}
			\def \k {9}
			\def \radius {18ex}
			\def \nodedist {.9ex}
			\def \margin {8} % margin in angles, depends on the radius
			\def \cliqueopacity {1} % opacity of cliques within components
			\def \labelposition {1.25} % distance of labels to the center
			\def \labelpositionC {.85}
	
			\draw (0,0) circle (\radius);
	

			\node[circle,draw,minimum size = 6.5*\nodedist,fill = white] (a_1) at ({360/\n * (2.5)}:\radius) {};
			\node[circle,draw,minimum size = 6.5*\nodedist,fill = white] (a_2) at ({360/\n * (0.5)}:\radius) {};
			\node[circle,draw,minimum size = 6.5*\nodedist,fill = white] (a_3) at ({360/\n * (8.5)}:\radius) {};
			\node[circle,draw,minimum size = 6.5*\nodedist,fill = white] (a_4) at ({360/\n * (6.5)}:\radius) {};
			\node[circle,draw,minimum size = 6.5*\nodedist,fill = white] (a_5) at ({360/\n * (4.5)}:\radius) {};
	
			\node[circle,draw,minimum size = 6.5*\nodedist,fill = white] (b_1) at ({360/\n * (1.5)}:\radius) {};
			\node[circle,draw,minimum size = 6.5*\nodedist,fill = white] (b_2) at ({360/\n * (9.5)}:\radius) {};
			\node[circle,draw,minimum size = 6.5*\nodedist,fill = white] (b_3) at ({360/\n * (7.5)}:\radius) {};
			\node[circle,draw,minimum size = 6.5*\nodedist,fill = white] (b_4) at ({360/\n * (5.5)}:\radius) {};
			\node[circle,draw,minimum size = 6.5*\nodedist,fill = white] (b_5) at ({360/\n * (3.5)}:\radius) {};
	
			\node[circle,draw,minimum size = 6.5*\nodedist] (c_1) at ($(a_1)!0.5!(b_4)$) {};
			\node[circle,draw,minimum size = 6.5*\nodedist] (c_2) at ($(a_2)!0.5!(b_5)$) {};
			\node[circle,draw,minimum size = 6.5*\nodedist] (c_3) at ($(a_3)!0.5!(b_1)$) {};
			\node[circle,draw,minimum size = 6.5*\nodedist] (c_4) at ($(a_4)!0.5!(b_2)$) {};
			\node[circle,draw,minimum size = 6.5*\nodedist] (c_5) at ($(a_5)!0.5!(b_3)$) {};
			
			
			\node at ({360/\n * (2.5)}:\radius*\labelposition) {$A_0$};
			\node at ({360/\n * (0.5)}:\radius*\labelposition) {$A_1$};
			\node at ({360/\n * (8.5)}:\radius*\labelposition) {$A_2$};
			\node at ({360/\n * (6.5)}:\radius*\labelposition) {$A_3$};
			\node at ({360/\n * (4.5)}:\radius*\labelposition) {$A_4$};	
			
			\node at ({360/\n * (1.5)}:\radius*\labelposition) {$B_0$};
			\node at ({360/\n * (9.5)}:\radius*\labelposition) {$B_1$};
			\node at ({360/\n * (7.5)}:\radius*\labelposition) {$B_2$};
			\node at ({360/\n * (5.5)}:\radius*\labelposition) {$B_3$};
			\node at ({360/\n * (3.5)}:\radius*\labelposition) {$B_4$};
			
			\node at ({360/\n * (2)}:\radius*\labelpositionC) {$C_0$};
			\node at ({360/\n * (10)}:\radius*\labelpositionC) {$C_1$};
			\node at ({360/\n * (8)}:\radius*\labelpositionC) {$C_2$};
			\node at ({360/\n * (6)}:\radius*\labelpositionC) {$C_3$};
			\node at ({360/\n * (4)}:\radius*\labelpositionC) {$C_4$};

	
			\foreach \x in {1,2,3,4,5}
			{
	
				\foreach \y in {1,2,3}
				{
					\node[circle,draw,position=42+120*\y-72*\x:{-2.7*\nodedist} from a_\x,opacity = \cliqueopacity] (a_\x\y) {};
					\node[circle,draw,position=54+42+120*\y-72*\x:{-2.7*\nodedist} from c_\x,opacity = \cliqueopacity] (c_\x\y) {};
			
				}
		
				\node[circle,draw,position=0-36+72-72*\x:{-2.7*\nodedist} from b_\x,opacity = \cliqueopacity] (b_\x1) {};
				\node[circle,draw,position=180-36+72-72*\x:{-2.7*\nodedist} from b_\x,opacity = \cliqueopacity] (b_\x2) {};
		
		
				\draw[opacity = \cliqueopacity] (a_\x1) -- (a_\x2);
				\draw[opacity = \cliqueopacity] (a_\x1) -- (a_\x3);	
				\draw[opacity = \cliqueopacity] (a_\x3) -- (a_\x2);
		
				\draw[opacity = \cliqueopacity] (c_\x1) -- (c_\x2);
				\draw[opacity = \cliqueopacity] (c_\x1) -- (c_\x3);	
				\draw[opacity = \cliqueopacity] (c_\x3) -- (c_\x2);
		
				\draw[opacity = \cliqueopacity] (b_\x1) -- (b_\x2);
		
			}
  
			\path[every node/.style={font=\sffamily\small}]
	
			(a_1) edge [near end] node {} (c_1) 
			(a_2) edge [near end] node {} (c_2) 
			(a_3) edge [near end] node {} (c_3) 
			(a_4) edge [near end] node {} (c_4) 
			(a_5) edge [near end] node {} (c_5) 
	
			(b_1) edge [near end] node {} (c_3) 
			(b_2) edge [near end] node {} (c_4) 
			(b_3) edge [near end] node {} (c_5) 
			(b_4) edge [near end] node {} (c_1) 
			(b_5) edge [near end] node {} (c_2) 
			
			\foreach \x in {1,2,3,4,5}
			{
			\foreach \y in {1,2,3,4,5}{
			(c_\y) edge [near end, dotted, darkgray] node {} (c_\x) 
			}
			}
			;

			\end{tikzpicture}

\caption{A simple and symmetric FHG with empty core. For all $j\in\{0,\dots,4\}$, $A_j$ and $C_j$ denote cliques of $3$ players and $B_j$ denotes a clique of $2$ players. An edge from one clique to another denotes that every player in the first clique is connected to every player in the second clique. All depicted edges have weight $1$. All missing edges have weight $0$. The example and the figure come from~\cite{Aziz14}. If the dotted edges are added between all the players in $\cup_j C_j$, we obtain a new instance with non-empty core.
}	\label{fig:fhg}
\end{figure}

\begin{comment}
(c_1) edge [near end] node {} (c_3) 
   (c_1) edge [near end] node {} (c_2) 
   (c_1) edge [near end] node {} (c_4) 
   (c_1) edge [near end] node {} (c_5) 
   (c_2) edge [near end] node {} (c_3)
   (c_2) edge [near end] node {} (c_4) 
   (c_2) edge [near end] node {} (c_5)
   (c_3) edge [near end] node {} (c_4) 
   (c_3) edge [near end] node {} (c_5)
   (c_4) edge [near end] node {} (c_5) 
\end{comment}


